Programmable EM Sensor Array for Golden-Model Free Run-time Trojan Detection and Localization

Side-channel analysis has been proven effective at detecting hardware Trojans in integrated circuits (ICs). However, most detection techniques rely on large external probes and antennas for data collection and require a long measurement time to detect Trojans. Such limitations make these techniques impractical for run-time deployment and ineffective in detecting small Trojans with subtle side-channel signatures. To overcome these challenges, we propose a Programmable Sensor Array (PSA) for run-time hardware Trojan detection, localization, and identification. PSA is a tampering-resilient integrated on-chip magnetic field sensor array that can be re-programmed to change the sensors' shape, size, and location. Using PSA, EM side-channel measurement results collected from sensors at different locations on an IC can be analyzed to localize and identify the Trojan. The PSA has better performance than conventional external magnetic probes and state-of-the-art on-chip single-coil magnetic field sensors. We fabricated an AES-128 test chip with four AES Hardware Trojans. They were successfully detected, located, and identified with the proposed on-chip PSA within 10 milliseconds using our proposed cross-domain analysis.

==> chatGPT_improve.tex <==
Hardware Trojans (HTs) are malicious circuits that are intentionally inserted into Integrated Circuits (ICs) during the design or fabrication process by an adversary. These HTs can have various objectives or "payloads," such as leaking protected information, causing denial of service, or escalating privileges. HTs can be active all the time or only when certain external or internal criteria, known as "triggers," are met. Triggers can be designed to evade detection during post-manufacturing tests.

The detection of HTs through the analysis of side-channel effects has been a topic of research for many years. Side-channel effects are signals, such as power consumption or electromagnetic (EM) emissions, that indirectly reveal information about the operations being performed on hardware. These effects can be detected after the chip has been fabricated, either during testing or at run-time. However, this process often requires specialized equipment and a reference model of a Trojan-free circuit. On-chip sensors, or sensors built into the IC design that can analyze side-channels at run-time, are therefore a preferred solution.

In previous work, He et al proposed a single coil that covers the entire chip area as a means of detecting HTs. However, this approach only allows for the detection of the presence of HTs on the chip and may not provide sufficient signal-to-noise ratio (SNR) for detecting all HTs. In addition, the single coil design is not able to localize HTs on the chip.

To address these limitations, we propose the Programmable Sensor Array (PSA). Our design, shown in Figure 1, consists of a crossbar-like structure with T-gates at each intersection, which are composed of parallel NMOS and PMOS transistors commonly used in VLSI design. The PSA can be programmed to change size and shape in order to include or exclude specific parts of the chip for improved SNR and HT localization. The size of individual sensors within the PSA can also be programmed to approximately match the size of a Trojan, allowing for the capture of the highest EM emissions from the HT. An op-amp can also be integrated on-chip to amplify the induced voltage signal measured by the PSA.

The main contributions of this paper are:

The proposal of the Programmable Sensor Array (PSA) as a means of detecting and localizing hardware Trojans (HTs)
The ability of the PSA to be programmed to change size and shape for improved signal-to-noise ratio (SNR) and HT localization
The integration of an op-amp on-chip to amplify the induced voltage signal measured by the PSA


There are several methods for detecting and analyzing electromagnetic (EM) side-channel leakage, which can be used to identify the presence of Hardware Trojans (HTs). Traditional EM side-channel approaches involve using an external EM probe, connected to an oscilloscope, to record the voltages induced on the probe above the package of an Integrated Circuit (IC). These recorded voltages can then be compared in the time or frequency domains to detect HTs. The probe is typically placed above the IC because the metal layers at the top of the design tend to be thicker than the layers at the bottom, resulting in stronger EM side-channel effects.

An alternative to this method is presented in a study by Nguyen et al., in which a transmitter antenna and a receiver antenna are placed on opposite sides of an IC to investigate the effects of HTs on the EM backscattering of the signal. The impedance changes caused by HT activity on the chip modulate the carrier signal emitted by the transmitter, which is captured by the receiver. While many HTs may have minimal effects on the current induced on external probes, their activation can significantly impact the carrier signal being sent towards the IC. On-chip EM sensors have also been studied, as seen in the work by He et al.

In this paper, we propose a new method called the Programmable Sensor Array (PSA), which can be used to detect and locate HTs. We compare the PSA technique to the three aforementioned families of approaches in Table I.

Researchers have developed a range of algorithms to analyze side-channel data for the purpose of detecting Hardware Trojans (HTs). Some examples include frequency spectrum analysis and Euclidean distance calculation of time-domain signals, as used in the work of He [4]. However, Euclidean distance analysis can require several thousands of traces to create a profile, which may not be practical at run-time due to the rarity of HT activation that escapes detection during the test phase [2].

Other approaches to side-channel analysis include the use of on-chip thermal sensors to track device temperature and identify spikes in power draw that may indicate HT activity [8]. This method uses a Kalman Filter's autocorrelation as a global anomaly detection approach to process data from multiple temperature sensors on a chip, and requires fewer data points than Euclidean distance methods. However, applying time-series filters in the EM domain requires complicated EM modeling of the circuits, making it difficult to implement on a VLSI design.

More recent approaches to side-channel analysis have utilized machine learning (ML) and deep learning (DL) techniques to improve performance. For example, convolutional neural networks (CNNs) have been shown to improve HT detection [9]. Nguyen's work [6] uses Principal Component Analysis (PCA) followed by a K Nearest Neighbor (KNN) unsupervised classification on the frequency spectrum to classify HT inactive and HT active cases. Similarly, Zhang et al. [10] use a classification algorithm to analyze frequency signals collected from a ring oscillator network (RON). Faezi et al. [5] use a CNN model to extract features most relevant to HT activation and classify HTs as inactive or active. The pros and cons of these data analysis methods are summarized in Table II.


% \section{Cross-domain HT Detection Technique} 

% In this paper, we introduce a pioneering cross-domain method for detecting and identifying HTs. We initially detect the Trojan through the spectrum analysis of the measured leakage magnetic field. Notably, when Trojans are active, they yield specific spectral signatures in the voltage readings of a PSA. By comparing the spectrum during inactive and active HT states, we can detect the presence of HTs. To further pinpoint these Trojans, we utilize a spectrum analyzer's zero-span mode, which provides a detailed view of magnitude changes over time for specific frequency signals.

% The zero-span mode facilitates a thorough investigation of the time-domain information of individual frequencies of interest. When comparing the time-domain waveform of a specific signature frequency with designs that have different active Trojans, we can identify the exact Trojan at play. Unlike traditional time-domain techniques that consider a combined waveform from all frequency components, our approach allows us to focus on individual frequencies. This specificity is essential as large amplitude non-significant frequencies can sometimes overshadow those carrying leakage signals from HTs in conventional methods.

% Traditional frequency-domain techniques usually detect the Trojan by contrasting the spectra from both inactive and active HT states. However, they often omit examining the time-domain information of individual frequency components responsible for HT leakage signals. This oversight can lead to missed detections. Our cross-domain approach fills this gap, providing a more comprehensive method for Trojan detection and identification.

% \begin{table}[]
%     \captionsetup{font={small, sc}}
%     \centering
%     \caption{Comparison of EM side-channel data analysis methods.}
%     \begin{tabular}{|p{2cm}|p{1.2cm}|p{0.9cm}|p{0.9cm}|p{1cm}|}
%         \hline 
%          \textbf{Features} &\textbf{Euclidean Distance} &\textbf{ML} & \textbf{DL} &\textbf{Cross-domain} \\
%          \hline\hline
%          Required Traces & High & Low & Medium & Low\\
%          \hline 
%          Sensitivity & Low & High & High & High \\
%          \hline
%          Label free & Yes & Yes & No & Yes \\
%          \hline
%          Accuracy & Low & Medium & High & High \\
%          \hline
%     \end{tabular}
%     \vspace{5pt}
    
%     \label{tab:data_compar}
% \end{table}
